Path-RAG: Knowledge-Guided Key Region Retrieval for Open-ended Pathology Visual Question Answering

Accurate diagnosis and prognosis assisted by pathology images are essential for cancer treatment selection and planning. Despite the recent trend of adopting deep-learning approaches for analyzing complex pathology images, they fall short as they often overlook the domain-expert understanding of tissue structure and cell composition. In this work, we focus on a challenging Open-ended Pathology VQA (PathVQA-Open) task and propose a novel framework named Path-RAG, which leverages HistoCartography to retrieve relevant domain knowledge from pathology images and significantly improves performance on PathVQA-Open. Admitting the complexity of pathology image analysis, Path-RAG adopts a human-centered AI approach by retrieving domain knowledge using HistoCartography to select the relevant patches from pathology images. Our experiments suggest that domain guidance can significantly boost the accuracy of LLaVA-Med from 38% to 47%, with a notable gain of 28% for H&E-stained pathology images in the PathVQA-Open dataset. For longer-form question and answer pairs, our model consistently achieves significant improvements of 32.5% in ARCH-Open PubMed and 30.6% in ARCH-Open Books on H\&E images. Our code and dataset is available here (https://github.com/embedded-robotics/path-rag).

==> Related_works.tex <==
% Feel free to delete some of this section because most MICCAI 2023 papers have very few related work parts even combine them into the introduction.
Pathology visual question-answering tasks will help facilitate diagnostic decisions in cancer. In this section, we first discuss existing work on open-ended pathology visual question answering, which traditionally addresses the problem by formulating open-ended questions as classification tasks, i.e., models generate predictions based on a predetermined pool of answers. Secondly, we review the research that formulates the task as a generation task (typically using multimodal LLMs) and discuss graph analytics in digital pathology, which has great potential in facilitating pathology VQA.
\subsubsection{Open-ended Pathology Visual Questions Answering: Formulated as Classification Task.} Path-VQA~\cite{he2020pathvqa} serves as a benchmark with 32,799 open-ended questions and answers from 4,998 pathology images in open-ended pathology VQA. Historically, in Path-VQA, while performance for open-ended questions has shown improvement, the LLaVA-Med~\cite{li2024llava} paper and CLIP-ViT w/ GPT2 (LORA)~\cite{van2023open} paper critique that most prior research 'overestimates their generalizability' as they 'formulate the problem as classification'. Below, we report on representative research that 'formulates the problem as classification'. MEVF~\cite{nguyen2019overcoming} employs MAML pre-trained weights and CDAE, leveraging BAN or SAN for integrated question-answer representation, achieving 8.1\% accuracy on PathVQA. MMQ~\cite{do2021multiple} develops an analogous embedding by leveraging annotations from various meta-models and meta-annotation training, reaching 11.8\% accuracy on PathVQA. K-PathVQA~\cite{Naseem2023-dg} uses a medical knowledge graph (KG) from a complementary external structured knowledge base to infer answers for the PathVQA task and achieved 42.12\% accuracy. This prior research predominantly formulates the open-ended pathology visual question-answering task as a classification task, typically using accuracy as the evaluation metric. However, this approach is suboptimal for the pathology dataset, as it typically involves answers that are already present in the training set, leading to inflated accuracy scores~\cite{li2024llava,van2023open}.
\subsubsection{Open-ended Pathology Visual Questions Answering: Formulated as Generation Task.} Highlighting the limitations mentioned in the LLaVA-Med~\cite{li2024llava} paper and previous sections, the standard formulation of open-ended pathology visual question answering as a classification task falls short. Van Sonsbeek et al.~\cite{van2023open} argued that language models are more suited for open-ended pathology VQA as the task is generative. They mapped the extracted visual features to a set of learnable tokens and then used the tokens and questions to prompt GPT-2, achieving 40.0\% accuracy. Q2ATransformer~\cite{Liu2023-rj} is a Transformer-based framework that enhanced accuracy to 54.85\%. Recent research shifts towards using recall as a metric to more accurately assess the completeness of free-form text responses in open-set scenarios. LLaVA-Med~\cite{li2024llava} was fine-tuned on a biomedical figure-caption dataset extracted from PubMed Central, using GPT-4 self-instruct open-ended instruction-following data from the captions. Of their three base models: LLaVA, Vicuna, and BioMed CLIP, LLaVA-Med (BioMed CLIP) achieved a 39.6\% recall (fine-tuned on PathVQA). Alongside LLaVA-Med~\cite{li2024llava}, there have been several studies focused on open-ended Pathology VQA using multimodal LLMs, e.g., Quilt-LLaVA~\cite{saygin2023quilt}, Med-Flamingo~\cite{moor2023medflamingo}. Quilt-LLaVA~\cite{saygin2023quilt} achieved a 15.30\% recall on PathVQA (not fine-tuned). In our PATH-RAG framework, we emphasize recall to evaluate how comprehensively the model's responses encompass ground-truth tokens for open-ended questions following~\cite{li2024llava}'s methodology. Though using multimodal LLMs has improved research performance and better conceptualized the task, the above methods did not use professional psychological tools to better answer open-ended questions. Our PATH-RAG framework incorporates the graph analytic tool HistoCartography~\cite{pmlr-v156-jaume21a}, which can significantly improve VQA performance on open-ended pathology questions. HistoCartography~\cite{pmlr-v156-jaume21a} is a toolkit for graph analytics in digital Pathology. It can generate nuclei graphs from pathology images. Thus, we can identify the most important patches in a pathology image. In the methodology section, we will specifically detail the application of HistoCartography~\cite{pmlr-v156-jaume21a} within our PATH-RAG framework to advance the open-ended VQA performance.

% The PathVQA paper~\cite{he2020pathvqa} uses traditional VQA methods and achieved a BLEU-1 of .32 and an F1 of .24. MedFuseNet~\cite{Sharma2021-xs} achieved a BLEU-1 of .61, BLEU-2 of .30, and F1 of 0.38.

==> Tables/effect_of_diff_components.tex <==
\begin{table}[htbp]
    \centering
    \caption{Ablation Study Results}
    \label{tab:ablation_study}
    \begin{tabular}{lccc}
        \toprule
        \textbf{Form} & \textbf{GPT-4}  & \textbf{Recall (H\&E-stained)} & \textbf{Recall (All)} \\
        \midrule
        Description & Yes & 
        % \begin{tabular}[t]{@{}p{5cm}@{}}You are a professional pathologist. Generate a comprehensive answer that integrates multiple perspectives for a pathology image, and provide a balanced conclusion based on the information provided.\\ Perspective 1: \\ Perspective 2: \\ Perspective 3: \\ Perspective 4: \\ Question: \end{tabular} 
        37.0 & 31.5 \\
        Answer & No & 36.4 & 38.1 \\
        Answer & Yes & 
        % \begin{tabular}[t]{@{}p{5cm}@{}}You are a pathologist examining a high-resolution medical image. You are tasked with providing detailed descriptions of different regions of interest (ROIs) within the image and relating these observations to answer the following question:\\ Image Description: \\ Patch 1 Description: \\ Patch 2 Description: \\ Patch 3 Description: \\ Question: \end{tabular} 
        \textbf{64.1} & \textbf{47.4} \\
        \bottomrule
    \end{tabular}
\end{table}

==> figure1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{image/conceptual figure.pdf}
    \caption{Conceptual Figure.}
    \label{fig:conceptual}
\end{figure}

==> introduction.tex <==
Pathology image analysis plays an essential role in the diagnosis, treatment, and study of cancer ~\cite{Wang2019-vm}. For example, reading hematoxylin and eosin (H\&E)-stained slides is a clinical standard of care for the diagnosis and staging of many cancers~\cite{Luo2017-jq}. The advent of whole-slide image (WSI) scanning, capable of capturing intricate histological details at high resolutions, has enabled remarkable advancements in pathology image analysis through deep learning algorithms to detect cancer regions~\cite{Kather2016-fn}, classify tissue subtypes~\cite{Javed2020-cg}, and identify diagnostically relevant structures and regions (e.g., nuclei~\cite{Gamper2019-fr}, glands~\cite{Graham2019-ux}, vessels and nerves~\cite{Fraz2020-dx}). Since pathology images are complex and tightly connected with different tissue structures, normal deep learning approaches, that typically involve patch generation, patch-level feature extraction, and feature aggregation to generate image-level embeddings for pathology tasks, fall short as they often overlook crucial tissue structure and cell composition~\cite{pmlr-v156-jaume21a}. The critical step for diagnosing pathology images is the pathologist’s ability to identify tissue structure and examine the cellular composition, organization, and architecture of tissues to characterize features of normal structures and abnormal cells in histologic sections~\cite{Bauer2020-ka}. Therefore, domain knowledge is critical for pathology imaging diagnosis, especially information related to tissue structure and cellular composition.

\input{figure2}

Cell graphs of cancer have been generated based on pathology images showing the distinct features compared with healthy cells at the cellular level and at the tissue level~\cite{Gunduz2004-ay}. Cell graphs are one kind of entity graph where nodes and edges of the graphs denote tissue entities and their interactions. The entities can be nuclei, tissue regions, and glands. Entity graphs can simultaneously capture local entity environment and global tissue composition, illustrating an ideal way to capture domain-specific knowledge in pathology images. Entity graphs can improve the efficiency in diagnosis considering that only diagnostically relevant entities have been analyzed, instead of analyzing the entire pathology images~\cite{Shaban2020-ny}. Generating entity graphs requires a complex workflow including stain normalization, tissue detection, entity detection, entity encoding, and constructing graph topology. HistoCartography is an open-source Python library that unifies a set of histology image manipulation tools to build entity graphs~\cite{Graham2019-ux,Ahmedt-Aristizabal2022-sa}, including stain normalization, tissue detection, nuclei detection, tissue component detection, feature extraction, and cell graph builders.

Open-ended Pathology visual question answering (VQA) is a challenging task with state-of-the-art methods achieving a recall of only 38\%~\cite{li2024llava}. These open-ended questions require a deep comprehension of both images and textual questions, and the relationship between visual objects and textual entities, especially the intricate domain knowledge in pathology. Therefore, identifying key regions in pathology images and retrieving relevant domain knowledge from the image is crucial to address challenges for open-ended pathology visual question answering. This paper introduces a framework, Path-RAG, which leverages HistoCartography to retrieve specific domain knowledge from pathology images, thereby enhancing the accuracy of open-ended visual question answering.

In addition to using LLaVA-MED fine-tuned on PathVQA~\cite{he2020pathvqa}, we construct a custom dataset consisting of open-ended question-answer pairs using the images and captions provided in ARCH~\cite{gamper2020multiple}

Our primary contributions can be summarized as:

\vspace{-0.3em}
\begin{itemize}
    \item[$\bullet$] \textbf{Significant Performance Improvement with up to 28\% increase in the recall.}
    Path-RAG is a human-centered AI approach by retrieving domain knowledge using HistoCartography to select the most relevant patches for a given pathology image, which can significantly boost the recall of LlaVa-Med for PathVQA Open-ended questions from 38\% to 47\%, especially with a significant improvement of 28\% for H\&E-stained pathology images;
    \vspace{0.1em}
    % \item[$\bullet$] \textbf{Consistent Performance using different methods.}
    % Path-RAG has demonstrated consistent performance when using LLaVa-Med to get the answer directly or using LLaVa-Med to generate descriptions of one image and its relevant patches as a prompt for GPT-4 to get the answer.
    \item[$\bullet$] \textbf{Consistent performance gain with and without GPT-4.} Path-RAG has demonstrated consistent performance benefits over LLaVa-Med for open-ended QA with and without GPT-4 component indicating the significance of domain guidance in pathology image analysis.
    \vspace{0.1em}
    \item[$\bullet$] \textbf{Performance improvement for non-finetuned LLaVa-Med.}
    Path-RAG can improve the recall by 12\% when using LLaVa-Med not finetuned on PathVQA to generate descriptions as a prompt for GPT-4 to get the answer on H\&E-stained slides.
\end{itemize}



% 1) Path-RAG is a human-centered AI approach by retrieving domain knowledge using HistoCartography to select the most relevant patches for a given pathology image, which can significantly boost the accuracy of LLaVA-Med for PathVQA Open-ended questions from 38\% to 43\%, especially with a significant improvement of 15\% for H\&E-stained pathology images; 2) Path-RAG has demonstrated the consistent performance when using LLaVA-Med to get the answer directly or using LLaVA-Med to generate descriptions of one image and its relevant patches as a prompt for GPT-4 to get the answer; 3) Path-RAG can improve the recall by 6\% when using LLaVA-Med not finetuned on PathVAQ to generate descriptions as a prompt for GPT-4 to get the answer on H\&E-stained pathology images.

